Measurement of three-jet production cross-sections in pp collisions at 7 TeV centre-of-mass energy using the ATLAS detector

Double-differential three-jet production cross-sections are measured in proton-proton collisions at a centre-of-mass energy of $\sqrt{s} = 7$ TeV using the ATLAS detector at the Large Hadron Collider. The measurements are presented as a function of the three-jet mass $(m_{jjj})$, in bins of the sum of the absolute rapidity separations between the three leading jets $(|Y^\ast|)$. Invariant masses extending up to 5 TeV are reached for $8< |Y^\ast| < 10$. These measurements use a sample of data recorded using the ATLAS detector in 2011, which corresponds to an integrated luminosity of 4.51 fb$^{-1}$. Jets are identified using the anti-$k_t$ algorithm with two different jet radius parameters, R=0.4 and R=0.6. The dominant uncertainty in these measurements comes from the jet energy scale. Next-to-leading-order QCD calculations corrected to account for non-perturbative effects are compared to the measurements. Good agreement is found between the data and the theoretical predictions based on most of the available sets of parton distribution functions, over the full kinematic range, covering almost seven orders of magnitude in the measured cross-section values.

==> auxiliary.tex <==
\clearpage
\section{Auxiliary Plots}


\begin{figure}[htp!]
\begin{center}
\includegraphics[width=0.45\linewidth]{Total_Syst_R06_ystar_00_20}
\includegraphics[width=0.45\textwidth]{Total_Syst_R06_ystar_20_40}  \\
\includegraphics[width=0.45\textwidth]{Total_Syst_R06_ystar_40_60}
\includegraphics[width=0.45\textwidth]{Total_Syst_R06_ystar_60_80} \\
\includegraphics[width=0.45\linewidth]{Total_Syst_R06_ystar_80_100}
\end{center}
\caption{
Total systematic uncertainty in the \trijet{} \xs{}  for \antikt{} \rsix{} jets as a function of \mjjj{}  in  $\ystar$ bins. The  bands shows the uncertainties due to jet energy scale, jet angular resolution, jet energy resolution and the combined uncertainty due to jet quality selection and unfolding. The outer band represents the total experimental uncertainty.
\label{fig:systematicsAll}
}
\end{figure}



\begin{figure}[hp!]
\begin{center}
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_0_2_jet0_jet1.pdf}
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_2_4_jet0_jet1.pdf}
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_4_6_jet0_jet1.pdf}\\
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_6_8_jet0_jet1.pdf}
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_8_10_jet0_jet1.pdf}
\end{center}
\caption{
The $\Delta R$ distribution between leading and subleading jets in \ystar{} bins for \rsix{} jet identified with \antikt{} algorithm.
Data are shown with black markers, where errors bars represent statistical uncertainty only.
The \pythia~6 with \perugia~2011 tune (\alpgen) predictions are plotted with blue (orange) lines.
The distributions are shown at the detector level.
}
\end{figure}


\begin{figure}[hp!]
\begin{center}
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_0_2_jet0_jet2.pdf}
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_2_4_jet0_jet2.pdf}
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_4_6_jet0_jet2.pdf}\\
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_6_8_jet0_jet2.pdf}
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_8_10_jet0_jet2.pdf}
\end{center}
\caption{
The $\Delta R$ distribution between leading and sub-subleading jets in \ystar{} bins for \rsix{} jet identified with \antikt{} algorithm.
Data are shown with black markers, where errors bars represent statistical uncertainty only.
The \pythia~6 with \perugia~2011 tune (\alpgen) predictions are plotted with blue (orange) lines.
The distributions are shown at the detector level.
}
\end{figure}

\begin{figure}[hp!]
\begin{center}
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_0_2_jet1_jet2.pdf}
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_2_4_jet1_jet2.pdf}
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_4_6_jet1_jet2.pdf}\\
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_6_8_jet1_jet2.pdf}
\includegraphics[width=0.32\columnwidth]{deltaR_R06_y_8_10_jet1_jet2.pdf}
\end{center}
\caption{
The $\Delta R$ distribution between subleading and sub-subleading jets in \ystar{} bins for \rsix{} jet identified with \antikt{} algorithm.
Data are shown with black markers, where errors bars represent statistical uncertainty only.
The \pythia~6 with \perugia~2011 tune (\alpgen) predictions are plotted with blue (orange) lines.
The distributions are shown at the detector level.
}
\end{figure}



\clearpage

\begin{figure}[hp!]
\begin{center}
\includegraphics[width=0.32\columnwidth]{pt_R06_y_0_2_jet0.pdf}
\includegraphics[width=0.32\columnwidth]{pt_R06_y_0_2_jet1.pdf}
\includegraphics[width=0.32\columnwidth]{pt_R06_y_0_2_jet2.pdf}\\
\includegraphics[width=0.32\columnwidth]{pt_R06_y_6_8_jet0}
\includegraphics[width=0.32\columnwidth]{pt_R06_y_6_8_jet1.pdf}
\includegraphics[width=0.32\columnwidth]{pt_R06_y_6_8_jet2.pdf}\\
\end{center}
\caption{
The \pt{} and rapidity distributions of the first three jets in $\ystar{}<2$ and $(6<\ystar<8)$ bins for \rsix{} jet identified with \antikt{} algorithm.
Data are shown with black markers, where errors bars represent statistical uncertainty only.
The \pythia~6 with \perugia~2011 tune (\alpgen) predictions are plotted with blue (orange) lines.
The distributions are shown at the detector level.
}
\end{figure}



\begin{figure}[hp!]
\begin{center}
\includegraphics[width=0.32\columnwidth]{rapidity_R06_y_0_2_jet0.pdf}
\includegraphics[width=0.32\columnwidth]{rapidity_R06_y_0_2_jet1.pdf}
\includegraphics[width=0.32\columnwidth]{rapidity_R06_y_0_2_jet2.pdf}\\
\includegraphics[width=0.32\columnwidth]{rapidity_R06_y_6_8_jet0}
\includegraphics[width=0.32\columnwidth]{rapidity_R06_y_6_8_jet1.pdf}
\includegraphics[width=0.32\columnwidth]{rapidity_R06_y_6_8_jet2.pdf}\\
\end{center}
\caption{
The \pt{} and rapidity distributions of the first three jets in $\ystar{}<2$ and $(6<\ystar<8)$ bins for \rsix{} jet identified with \antikt{} algorithm.
Data are shown with black markers, where errors bars represent statistical uncertainty only.
The \pythia~6 with \perugia~2011 tune (\alpgen) predictions are plotted with blue (orange) lines.
The distributions are shown at the detector level.
}
\end{figure}

% \includegraphics[width=0.32\columnwidth]{plots/Kinematic_perjet/pdf/pt_R04_y_0_2_jet0.pdf}
% \includegraphics[width=0.32\columnwidth]{plots/Kinematic_perjet/pdf/pt_R04_y_2_4_jet0.pdf}
% \includegraphics[width=0.32\columnwidth]{plots/Kinematic_perjet/pdf/pt_R04_y_4_6_jet0.pdf}\\
% \includegraphics[width=0.32\columnwidth]{plots/Kinematic_perjet/pdf/pt_R04_y_6_8_jet0.pdf}
% \includegraphics[width=0.32\columnwidth]{plots/Kinematic_perjet/pdf/pt_R04_y_8_10_jet0.pdf}

\clearpage


\begin{figure}[htp!]
\centering
  \includegraphics[width=.45\linewidth]{result_h_trijet_Mass_AKT04_YS0}
  \includegraphics[width=.45\linewidth]{result_h_trijet_Mass_AKT04_YS1}\\
  \includegraphics[width=.45\linewidth]{result_h_trijet_Mass_AKT04_YS2}
  \includegraphics[width=.45\linewidth]{result_h_trijet_Mass_AKT04_YS3}  \\
  \includegraphics[width=.45\linewidth]{result_h_trijet_Mass_AKT04_YS4}
\caption{
\label{fig:npcorrAll4}
Non-perturbative corrections  obtained using various MC generators and tunes are shown for the differential \trijet{} \xs{} as a function of \trijet{} mass in the range $\ystar<10$ with values of jet radius parameter \rfour. The non-perturbative correction uncertainty is taken  as the envelope of the various tunes.
}

\end{figure}
\begin{figure}[htp!]
\centering
  \includegraphics[width=.45\linewidth]{result_h_trijet_Mass_AKT06_YS0}
  \includegraphics[width=.45\linewidth]{result_h_trijet_Mass_AKT06_YS1}\\
  \includegraphics[width=.45\linewidth]{result_h_trijet_Mass_AKT06_YS2}
  \includegraphics[width=.45\linewidth]{result_h_trijet_Mass_AKT06_YS3}  \\
  \includegraphics[width=.45\linewidth]{result_h_trijet_Mass_AKT06_YS4}
\caption{
\label{fig:npcorrAll6}
Non-perturbative corrections  obtained using various MC generators and tunes are shown for the differential \trijet{} \xs{} as a function of \trijet{} mass in the range $\ystar<10$ with values of jet radius parameter \rsix. The non-perturbative correction uncertainty is taken  as the envelope of the various tunes.
}
\end{figure}





\clearpage

   \begin{figure}
     \centering
\includegraphics[width=0.48\columnwidth]{bands_threejets_R4_00_20_CT10nlo}
\includegraphics[width=0.48\columnwidth]{bands_threejets_R4_20_40_CT10nlo}
\includegraphics[width=0.48\columnwidth]{bands_threejets_R4_40_60_CT10nlo}
\includegraphics[width=0.48\columnwidth]{bands_threejets_R4_60_80_CT10nlo}
\includegraphics[width=0.48\columnwidth]{bands_threejets_R4_80_100_CT10nlo}
     \caption{Relative uncertainties on NLO pQCD predictions as a function of \mjjj{} in bins of
   \ystar{} using CT10 PDFs for \rfour{} \antikt{} jets. The \xs{} variation, $\Delta\sigma$, with respect to the central values of
   the prediction, $\sigma_0$, are shown as a ratio to the central values. The uncertainties due to the PDFs, the choices of renormalisation
   and factorisation factors and the $\alpha_s$ value are shown.}
     \label{fig:nloct10_1_r4}
   \end{figure}


   \begin{figure}
     \centering
\includegraphics[width=0.48\columnwidth]{bands_threejets_R6_00_20_CT10nlo}
\includegraphics[width=0.48\columnwidth]{bands_threejets_R6_20_40_CT10nlo}
\includegraphics[width=0.48\columnwidth]{bands_threejets_R6_40_60_CT10nlo}
\includegraphics[width=0.48\columnwidth]{bands_threejets_R6_60_80_CT10nlo}
\includegraphics[width=0.48\columnwidth]{bands_threejets_R6_80_100_CT10nlo}
     \caption{Relative uncertainties on NLO pQCD predictions as a function of \mjjj{} in bins of
   \ystar{} using CT10 PDFs for \rsix{} \antikt{} jets. The \xs{} variation, $\Delta\sigma$, with respect to the central values of
   the prediction, $\sigma_0$, are shown as a ratio to the central values. The uncertainties due to the PDFs, the choices of renormalisation
   and factorisation factors and the $\alpha_s$ value are shown.}
     \label{fig:nloct10_1_r6}
   \end{figure}


       \clearpage
\endinput



